Cellular Automata: Reversibility, Semi-reversibility and Randomness

In this dissertation, we study two of the global properties of 1-dimensional cellular automata (CAs) under periodic boundary condition, namely, reversibility and randomness. To address reversibility of finite CAs, we develop a mathematical tool, named reachability tree, which can efficiently characterize those CAs. A decision algorithm is proposed using minimized reachability tree which takes a CA rule and size n as input and verifies whether the CA is reversible for that n. To decide reversibility of a finite CA, we need to know both the rule and the CA size. However, for infinite CAs, reversibility is decided based on the local rule only. Therefore, apparently, these two cases seem to be divergent. This dissertation targets to construct a bridge between these two cases. To do so, reversibility of CAs is redefined and the notion of semi-reversible CAs is introduced. Hence, we propose a new classification of finite CAs -(1) reversible CAs, (2) semi-reversible CAs and (3) strictly irreversible CAs. Finally, relation between reversibility of finite and infinite CAs is established. This dissertation also explores CAs as source of randomness and build pseudo-random number generators (PRNGs) based on CAs. We identify a list of properties for a CA to be a good source of randomness. Two heuristic algorithms are proposed to synthesize candidate (decimal) CAs which have great potentiality as PRNGs. Two schemes tare developed o use these CAs as window-based PRNGs - (1) as decimal number generators and as (2) binary number generators. We empirically observe that in comparison to the best PRNG SFMT19937-64, average performance of our proposed PRNGs are slightly better. Hence, our decimal CAs based PRNGs are one of the best PRNGs today.

==> CHANGES <==
glossaries change log:

v4.42 (2019-01-06):

 * glossaries.sty:

  - changed \edef to \protected@csedef in \glsfieldedef

  - changed \xdef to \protected@csxdef in \glsfieldxdef

  - added package option 'noglossaryindex' to counteract 'index'
    (if 'index' happens to be supplied as a global option)

  - automake option now takes 'immediate' as a value.

 * glossary-longbooktabs.sty:

  - removed superfluous \glspatchLToutput

v4.41 (2018-07-23):

 * glossaries.sty:

  - added package option kernelglossredefs (Warnings are now
    generated if the kernel commands \makeglossary and \glossary are
    used. These commands are deprecated with the glossaries package.
    If the originals are required, by a package or class that must
    be used with glossaries.sty for some reason, then use 
    kernelglossredefs=false, but beware of other possible conflicts.)

  - renamed some internal commands to avoid conflict
     \gls@debug@val, \gls@debug@nr
     \gls@seenoindex@val, \gls@seenoindex@nr
     \gls@numberedsection@val, \gls@numberedsection@nr
     \gls@translate@val, \gls@translate@nr
     \gls@nonumberlist@val, \gls@nonumberlist@nr

v4.40 (2018-06-01):

 * bug fix: corrected page number reference when
   using \makenoidxglossaries 

v4.39 (2018-05-23):

 * makeglossaries-lite.lua:

  - corrected version information

 * glossariesbegin.tex:

  - updated further information section

 * glossaries-user.tex:

  - updated some external links

v4.38 (2018-05-10):

 * glossaries.sty:

  - added \GlsEntryCounterLabelPrefix

  - bug fixes:

    - moved conditional inside \glsstepentry,
      \glsstepsubentry, \glsrefentry,
      \glsentrycounterlabel, \glssubentrycounterlabel, \glsentryitem,
      \glssubentryitem, \glsresetentrycounter, \glsresetsubentrycounter

    - removed spurious space in subentrycounter (printgloss) key

    - fixed use of entrycounter and subentrycounter in \setupglossaries

 * glossaries-accsupp.sty:

  - bug fixes:

   - added braces around argument of ActualText in \glsaccsupp

   - corrected field used in \showglonameaccess

v4.37 (2018-04-07):

 * glossaries.sty:

  - added \gls@begindocdefs

v4.36 (2018-03-07):

 * glossaries.sty:

  - bug fix (if \makeindex is used without \makeglossaries, 
    corrupted glossary information is written to the .idx file)

 * makeglossaries-lite.lua:

  - corrected check for double-quotes in \@istfilename
    (from \jobname when the .tex file name contains spaces)

  - added check for nil codepage

v4.35 (2017-11-14):

 * glossaries.sty:

  - bug fix (\glsadd breaks with sort=use)

v4.34 (2017-11-03):

 * glossaries.sty:

  - modified \glsshowtarget to check for math mode and inner

 * glossary-mcols.sty:

  - removed spurious space in mcolalttreespannav style

 * makeglossaries and makeglossaries-lite.lua:

  - added check for \glsxtr@resource

v4.33 (2017-09-20):

 * Removed makeglossaries.bat (TeX distributions on Windows
   convert the Perl script to makeglossaries.exe, so the
   .bat file isn't needed.)

 * makeglossaries and makeglossaries-lite.lua now have their
   version numbers synchronised with glossaries.sty

 * Added makeglossaries-lite.pod (to provide the
   makeglossaries-lite.1 man file)

 * Updated POD at the end of makeglossaries

 * Added example-glossaries-symbolnames.tex for use in any MWE 
   requiring symbols in the name fields.

 * Tidied up the user manual and guide for beginners.

 * glossaries.sty:

  - added package option nolangwarn

  - added package option esclocations

  - added \GlsSetXdyNumberGroupOrder

  - added starred form of \GlsSetXdyFirstLetterAfterDigits

v4.32 (2017-08-24):

 * glossaries.sty:

  - added debug=showtargets and associated commands
    \@glsshowtarget and \glsshowtarget

 * glossary-hypernav.sty:

  - added \@glsnavhypertarget

v4.31 (2017-08-10):

 * glossaries.sty:

  - Bug fix: 'nolist' option sets default style to \relax
    if currently set to 'list' to prevent trying to set an
    undefined style.

v4.30 (2017-06-11):

  * glossaries.sty:

   - Added sort=none option

   - Added \glosortentrieswarning

   - Added \@glo@autosee

   - Fixed bug occurring with \setupglossaries{sort=def}

   - Fixed bug in \@xdyuserlocationnames

   - Fixed bug in \@xdylocationclassorder

   - Added \@xdycrossrefhook

   - Added \@glo@check@sortallowed

   - Fixed bug in \printnoidxglossary with group skips in
     tabular styles

  * makeglossaries v2.21:

    - Fixed spelling mistake in warning message
      (\GlsAddLocation -> \GlsAddXdyLocation)

    - Adjusted range encap clash correction

v4.29:

  * glossaries-accsupp.sty: corrected check for glossaries-extra
    'accsupp' option.

  * glossaries.sty: moved definition of \@gls@currentlettergroup
    before \begin{theglossary} and made redefinitions of it within
    theglossary global to guard against scoping issues cause by
    tabular-like glossary styles.

  * glossary-hypernav.sty: added \glsnavhyperlinkname

v4.28:

  * glossaries.sty: added \glspatchtabularx

v4.27:

  * Version number updated in *.sty files, but no actual code
    change.

  * makeglossaries v2.20 and makeglossaries-lite.lua v1.3:

    - Added check for \glsxtr@makeglossaries

v4.26:

  * glossaries.sty:

    - added check for classicthesis.sty (if it's been loaded
      the default style is changed to "index" since the "list"
      style doesn't work with classicthesis.)

  * glossary-tree.sty:

    - new commands \glstreeitem, \glstreesubitem and
      \glstreesubsubitem provided for the "index" style
      to make the style easier to adjust.

    - replaced hard-coded \space with \glstreepredesc 
      or \glstreechildpredesc for all glossary-tree styles
      except for the alttree* styles.

  * glossary-mcol.sty:

    - The "mcolindex" and "mcolindexspannav" styles
      use the new \glstreeitem, \glstreesubitem and
      \glstreesubsubitem provided by glossary-tree.sty.

v4.25:

  * glossaries.sty:

    - bug fix
      http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=111

v4.24:

  * glossaries.sty:

    - added debug and seenoindex option

    - added \GlsSetWriteIstHook and \GlsSetQuote

    - added \@gls@extramakeindexopts for makeglossaries
      and makeglossaries-lite.lua (allow makeindex -g
      for German documents)

  * makeglossaries (2.19):

    - Improved check in &parse_for_xindy_nosort

    - Added check for \@gls@extramakeindexopts

  * makeglossaries-lite.lua (1.2):

    - Added check for nil codepage

v4.23

  * glossaries.sty:

    - added \glscurrentfieldvalue

  * tabular-like styles (glossary-long.sty etc):

    - bug fix (nogroupskip in tabular styles with "noidx" commands)
      http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=108

v4.22:

  * glossaries.sty:

    - added \gls@arabicpage

    - added \ifglswrallowprimitivemods

    - added \glsentrytitlecase

  * glossary-tree.sty:

    - new formatting commands \glstreegroupheaderfmt
      and \glstreenavigationfmt to
      make it easier to customize styles

    - new command \glsfindwidesttoplevelname

  * glossary-mcols.sty:

    - hard-coded \textbf replaced with
      \glstreegroupheaderfmt or \glstreenavigationfmt,
      as appropriate

    - added new styles mcolindexspannav, mcoltreespannav,
      mcoltreenonamespannav, mcolalttreespannav

  * glossary-list.sty:

    - new formatting commands \glslistgroupheaderfmt
      and \glslistnavigationitem to make it easier to 
      customize styles

    - fixed missing space before description in list
      style sub-entries.

  * glossary-super.sty:

    - fixed bug in super4col style

  * glossary-long.sty:

    - fixed bug in long style (typo in \glossentrydesc
      for sub-entries)

v4.21:

  * glossaries.sty:

    - Added warning if there's no default style.

  * glossary-longbooktabs.sty - new package

  * makeglossaries (2.18):

    - Added extra diagnostic if xindy's empty index key
      warning/error occurs.

    - Added check for makeindex's multiple encap warning
      and attempt to fix.

  * glossaries-user.tex:

    - Fixed typo: \DefineAcronymShortcuts should be
      \DefineAcronymSynonyms

v4.20:

  * makeglossaries (2.17) bug fix
   http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=101

  (No changes to any of the *.sty files, except the version number.)

v4.19:

  * glossaries.sty:

    - Added commands: \glsdoifexistsordo, 
      \doifglossarynoexistsordo 

    - Added some new internals that will be used by pending new
      package glossaries-extra.sty

  * glossary-tree.sty:

    - Added \glstreenamebox

v4.18:

  * mfirstuc removed from glossaries bundle and now
    needs to be installed separately

v4.17:

  * makeglossaries-lite.lua:

    - changed #! line "lua" to "texlua"

  * mwe-acr.tex and mwe-acr-desc.tex:

    - fixed misplaced \setacronymstyle

v4.16:

  * Added makeglossaries-lite.lua (Lua trimmed-down alternative 
    to Perl makeglossaries script. Doesn't have the full
    functionality of makeglossaries but doesn't require Perl.)

  * makeglossaries (Perl script):

    - fixed ngerman din5007 issue.

  * glossaries.sty:

    - new field-related commands:
      \glsaddstoragekey, \glsfielddef, \glsfieldedef,
      \glsfieldgdef, \glsfieldxdef, \glsfieldfetch,
      \ifglsfieldeq, \ifglsfielddefeq, \ifglsfieldcseq

    - new user command \glswriteentry to hook into mechanism
      that writes entry information to the external files

    - new user command \glspostlinkhook to hook into end of
      commands like \gls and \glstext.

    - Added new acronym styles "long-sp-short" and
      "long-sp-short-desc"

    - bug fix: \glsadd should use \@@do@wrglossary not
      \@do@wrglossary

v4.15:

  * glossaries.sty:

   - bug fix
     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=79

v4.14:

  * glossaries.sty:

    - Added \glsenableentrycount and associated commands
      and accompanying sample file sample-entrycount.tex 
      that illustrates them.

v4.13:

  * glossaries.sty:

    - provide a definition of \indexspace if not already defined
      for those styles that need it.

  * mfirstuc.sty (v1.10):

    - added \ecapitalisewords, \emakefirstuc

v4.12:

  * glossaries.sty:

    - Separated language-dependent code into separate
      modules to be independently installed, as required.

    - Fixed bugs:
      www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=67
      www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=69
      www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&category=glossaries&key=72

v4.11:

  * glossaries.sty:

    - Added \glsaddprotectedpagefmt

    - Put back the redefinition of \glossary (so that it takes an
      optional argument) removed in the previous version to 
      allow for packages that have hacked the internal glossary
      writing mechanism. (This may be removed or moved to a 
      compatibility mode in the future.)

    - Fixed backward compatibility support of deprecated
      sanitize=none option

    - Fixed bug introduced in v4.10 that caused a conflict with
      doc.sty

v4.10:

  * Added test file example-glossaries-url.tex 

  * glossaries.sty:

    - Added \glspercentchar and \glstildechar

    - Fixed problem with \Glsentryname (and \Glsname)
      when used with \setacronymstyle

    - No longer redefine \glossary but instead define
      a replacement internal command \gls@glossary, and 
      renamed \@glossary to \@gls@glossary

  * glossary-tree.sty:

    - Corrected location of space in alttree style with symbols

v4.09:

  * Fixed bug in \glsaddkey introduced in v4.08
    www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=64

v4.08:

  * New files: example-glossaries-*.tex

    These contain lorem ipsum dummy entries for testing
    new styles or constructing MWEs that require a lot of sample entries
    (to be placed on TeX's path)

  * glossaries.sty

   - new package option: automake

   - \newglossary now has a starred version where you don't need
     to specify the extensions

   - new commands: \forallacronyms, \newignoredglossary

   - new keys for \printglossary/\printnoidxglossary:
     entrycounter, subentrycounter, nopostdot

   - \gls etc now have a +-version (opposite of the *-version)
     that explicitly switches on the hyperlink with hyper=true
     (unlike the unstarred version that uses the default setting).

   - new commands for use within \glsentryfmt or \defglsentryfmt:
     \glsifhyperon and \glslinkvar (\glsifhyper now deprecated).

   - fixed bug that didn't correctly honour the hyper setting
     in commands like \glslink, \gls, glstext, etc under 
     certain situations.

   - fixed bug
     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=54

   - added \@gls@hyp@opt and removed now-redundant internal commands

   - removed some of the redundancy in commands like \gls

  * glossary-longragged.sty:

   - Fixed bug in altlongragged4col style that displayed the
     description instead of the symbol in the third column.

  * glossary-tree.sty:

   - Added \glstreenamefmt

  * mfirstuc.sty v1.09:

   - Added \MFUnocap

  * New package: mfirstuc-english.sty

  * makeglossaries

   - Fixed bug report
     http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=55

v4.07:

  * glossaries.sty:

   - Added \glsletentryfield

   - Bug fixes:
     - added optional argument to unstarred sectioning
       commands (used with package options numberedsection=nolabel
       and numberedsection=autolabel)

     - added \global prefix to definition of \@gls@loclist
       in \@gls@noidx@do in case a tabular-like style is used.

     - Fixed no case change bug in \Acrfullplfmt

v4.06:

  * glossaries.sty:

   - Added \glsifhyper

   - Fixed bookmark issue occurring with
     "numbers" and "symbols" package options
     in combination with hyperref.sty and translator.sty

v4.05:

  - Added missing glossaries-prefix.sty to tds

v4.04:

  * glossaries.sty:

   - new commands: \makenoidxglossaries, \printnoidxglossary
     and \printnoidxglossaries that use TeX to sort entries 
     instead of makeindex/xindy

   - new command: \glsnumberlistloop (for use with
     \makenoidxglossaries)

   - new package option: noredefwarn

   - moved definition of \glswrite to \makeglossaries so that write
     register is only allocated if required.

   - fixed bug in \defglsdisplayfirst

  * glossary-tree.sty:

   - fixed bug in alttree style


  * glossaries-accsupp.sty:

   - \compatibleglossentry and \compatiblesubglossentry:
     changed \newcommand to \def as they may or may not be
     defined depending on whether user has loaded glossaries
     separately from glossaries-accsupp

  * makeglossaries:

   - added -Q and -k switches

   - added extra diagnostics

v4.03:

  glossaries.sty:

   * Added \glsifhasfield

   * Changed default definition of \glswritefiles to \@empty
     instead of \relax

   * Fixed bug in \ifglsdescsuppressed

   * Added \glsdetoklabel

   * Added \glsdoifexistsorwarn

   * Changed \glossentryname etc to use \glsdoifexistsorwarn
     instead of \glsdoifexists

   * Added \renewacronymstyle

   * Fixed bug in dua acronym style

  glossaries-accsupp.sty:

   * Redefined acronym styles to use accessibility support

  makeglossaries v2.12:

   * Added check for backslashes in -x, -m and -d arguments


v4.02:

  glossaries.sty:

   * Added nameref value to 'numberedsection' package option

   * New package option: "index"

   * New package option: xindynoglsnumbers (equivalent to 
     xindy={glsnumbers=false})

   * Added \newacronymstyle, \setacronymstyle and associated
     commands. (Package options "smallcaps", "smaller",
     "description", "dua" and "footnote" now deprecated.)

   * New commands \acrfullfmt etc to govern the format of 
     \acrfull etc.

   * Made \makeglossaries preamble only

   * Bug Fixes:

     - \acrlong, \Acrlong, \ACRlong, \acrlongpl,
       \Acrlongpl and \ACRlongpl: removed \acronymfont and
       spurious parenthetical text.

     - \glsentryfull, \Glsentryfull, \glsentryfullpl,
       and \Glsentryfullpl: added missing \acronymfont

     - Fixed bug in "sanitize" package option (deprecated option,
       but still kept for backward compatibility).

v4.01:

  * Fixed bug in \CustomAcronymFields caused by missing comma.

  * Fixed valueless package options so that they can be passed via
    the document class.

v4.0:

  First stable release since v3.07.

v3.14a:

  * glossaries.sty

    - New package options: acronyms, xindygloss, notranslate

    - Modified savewrites option so that it can be set via
      \setupglossaries

    - Enabled compatible-3.07 option in \setupglossaries

    - Added \provideglossaryentry and \longprovideglossaryentry

    - Bug fix: fixed the default firstplural value to the value of
      the plural key.

  * glossaries-prefix.sty

    - New

  * makeglossaries v2.09:

    - added check for -q switch when issuing warnings

v3.13a:

  * glossaries.sty

    - Added \glsprestandardsort

    - Renamed \glossarymark to \glsglossarymark to prevent clash
      with memoir.

    - Made "translate" package option a choice key rather than boolean

    - Bug fix for \glsaddallunused: 
        set default value of optional argument to \@glo@types

    - Bug fix for \SetFootnoteAcronymDisplayStyle:
        added missing final argument of \ifglshaslong

    - Bug fix for \glossarystyle:
        replaced \ifdef with \ifcsdef

  * mfirstuc.sty (v1.08):

    - Made \makefirstuc and \capitalisewords robust

v3.12a:

  * glossaries.sty

    - Added \glsaddkey (allows the user to add their own custom 
      keys to glossary entries).

v3.11a:

  * glossaries.sty

    - Added \setupglossaries
      (http://www.dickimaw-books.com/cgi-bin/featuretracker.cgi?action=view&key=7)

    - Added \glsentryfmt and \defglsentryfmt
      and deprecated \glsdisplayfirst, \glsdisplay,
      \defglsdisplayfirst and \defglsdisplay
      (http://www.dickimaw-books.com/cgi-bin/featuretracker.cgi?action=view&key=13)

    - Added \longnewglossaryentry

    - Added \ifglshasshort and \ifglshaslong

    - Added check in \glsgetgrouptitle for non-Latin characters

    - Added compatible-3.07 package option

    - Added "symbols" and "numbers" package options
      (http://www.dickimaw-books.com/cgi-bin/featuretracker.cgi?action=view&key=16)

    - Added \printacronyms[opts] as a synonym for
      \printglossary[type=\acronymtype,opts]
      if "acronym" package option is used and
      "compatible-3.07" package has not been used
      and \printacronym doesn't already exist at the start
      of the document.

    - Added \showgloshort and \showglolong

    - Fixed bug in \@gls@noexpand@fields

    - Fixed bug in \gls@defglossaryentry that didn't set the default
      counter correctly

    - Now uses \mfirstucMakeUppercase instead of \MakeUppercase
      to be consistent with mfirstuc.

    - Now requires textcase (better handling of case changes)

  * mfirstuc (v1.07)

    - Added \mfirstucMakeUppercase to allow the user to switch from
      \MakeUppercase to another case changing command.

  * makeglossaries (v2.08)

    - Added -x and -m switches

v3.10a:

  * glossaries.sty

    - Added \providecommand to aux file in case user removes 
      the glossaries package from their document. (This ensures
      the next run doesn't throw a load of undefined control
      sequence errors when the aux file is parsed.)

    - Fixed new code (from v3.08a) so that document can still
      compile if entries are defined within the document after
      \printglossary or \printglossaries

v3.09a:

  * glossaries.sty

    - Added fix for \RecordChanges if doc.sty has been loaded

    - Fixed noexpand for symbolplural field
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=41)

    - Made \Glsentryname, \Glsentrytext etc robust

    - Fixed bug in footnote option
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=37)

    - Fixed bug where acronym starts with repeated letter
      (www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=34)

    - Added \glstextup which checks for \textulc
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=40)

v3.08a:

  * glossaries.sty

    - Changed the way information is written to external glossary
      files. Information is now written as just \glossentry{label}
      or \subglossentry{level}{label} instead of
      \glossaryentryfield{label}{name}{description}{symbol} or 
      \glossarysubentryfield{level}{label}{name}{description}{symbol} 
      This means that descriptions can span multiple paragraphs
      without exceeding makeindex's buffer.

    - Added \setglossarystyle (replaces \glossarystyle which is now
      just for backward compatibility)

    - New user commands: 

        \glossentryname, \Glossentryname,
        \glossentrydesc, \Glossentrydesc,
        \glossentrysymbol, \Glossentrysymbol,
        \glsexpandfields, \glsnoexpandfields,
        \glsaddallunused,
        \ifglshassymbol, ifglshasdesc

    - Added nogroupskip option to \printglossary

    - Added \gls@ifnotmeasuring

    - Made \glsseeformat, \glsseelist, \glsseeitem and \glssee robust

  * glossary-tree.sty

    - Added \par to end of theglossary environment for index style.
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=38)

v3.07:

  * glossaries.sty

    - Fixed bug relating to nohypertypes list option

    - Added \setglossarypreamble (code provided by Michael Pock)

    - Modified \glspostdescription to adjust spacefactor before full
      stop. (Patch provided by Michael Pock.)

    - Added check for openright in \gls@doclearpage

    - Added \glsdoparenifnotempty

    - Made \findrootlanguage obsolete

makeglossaries:

    - Added languagemap to determine root language

v3.06:

  * glossaries.sty

    - Fixed incompatibility between glossaries and new version of babel.

  * makeglossaries

    - added babel dialect -> xindy language map

v3.05:

  * glossaries.sty

    - fixed bugs related to location numbering (Roman and Alph).

    - made \nopostdesc robust

    - clarified in the documentation that \makeglossaries must be
      used before cross-referenced entries

    - added missing 'nohypertypes' code

  * makeglossaries:

    - added "din5007" as the default to makeglossaries if the
      language is german

  * glossary-mcols.sty:

    - Fixed bug -> \begin{multicols}{2} replaced with \begin{multicols}{\glsmcols}

v3.04:

  * added 'nohypertypes' package option

  * added new commands: \GlsDeclareNoHyperList and \glsIfNoHyperType

  * added 'local' key to \glsdisp, \gls, \Gls and \GLS

  * added check for doc package

  * fixed bug in altlist that can cause an unintentional page break
    between entry and description.

  * fixed bug that causes extra space after glossary when using
    xindy

  * fixed bug that was introduced by the bug fix in 3.02 regarding wrong
    page number

  makeglossaries v2.05:
  * added -d option

v3.03:

  * fixed bug in \printglossary options: title now also sets
    toctitle if toctitle missing (as per documentation).

  * added sanitize={sort=false} option

  * added nopostdot package option

  * added nogroupskip package option

   glossary-inline.sty added:

   - \glsinlinenameformat
   - \glsinlinedescformat
   - \glsinlineemptydescformat
   - \glsinlinesubnameformat
   - \glsinlinesubdescformat
   - \glsinlinepostchild

v3.02:

  * new package options:

    - 'ucmark'
    - 'indexonlyfirst'
    - 'savenumberlist'

  * new glossary styles:

    - glossary-mcol.sty
    - glossary-inline.sty

  * new commands:

    - \glolinkprefix
    - \glsmoveentry
    - \renewglossarystyle
    - \ifglshaschildren
    - \ifglshasparent
    - \glsresetentrycounter
    - \glsentrynumberlist
    - \glsdisplaynumberlist

  * added check to \glswritefiles to see if glossary tokens have
    been defined in case savewrites option used and \makeglossaries
    omitted.

  * fixed bug in \showglossaryentries

  * fixed bug in \SmallNewAcronymDef

  * fixed unwanted space in
    \SetDescriptionFootnoteAcronymDisplayStyle

  * fixed [xindy] wrong page number bug for entries occurring in
    paragraph spanning page break

  * fixed bug in \Glsentryfull and \glsentryfullpl

  * swapped order of checks for babel and polyglossia

  mfirstuc v1.06:

  * added \capitalisewords, \xcapitalisewords

  makeglossaries v2.04:

  * fixed bug in &scan_aux

v3.01:

   * made commands like \glslink, \gls and \acrshort robust

   * Fixed bugs in commands like \acrfullpl which was missing the
     plural in some cases.

   * Removed \acronymfont from \acrfullformat as it's already used
     in the second argument passed to that command. (Causes a 
     problem with the "smaller" option.)

v3.0 (Major changes):

   * Documentation has been restructured:

     - glossaries-user: main user manual
     - glossariesbegin: cut-down introduction for beginners
     - mfirstuc-manual: user manual for mfirstuc package
     - glossaries.pdf: documented code for advanced users
     - glossary2glossaries: upgrading from glossary.sty to glossaries.sty

   * Added new package options:

     - entrycounter : number main (level 0) entries in the glossary.

     - counterwithin : set parent counter for the entry counter.

     - subentrycounter : number level 1 entries in the glossary.

     - sort : set the sort order to 
              - standard alphabetical (sort=standard),
              - order of definition (sort=def) 
              - order of use (sort=use)

     - seeautonumberlist : automatically activates the number list
                           for entries that use the "see" key.

     - savewrites : minimise number of \newwrite

     - compatible-2.07 :

         bug fixes in v3.0 have cause compatibility problems. This 
         package option will restore the old behaviour but bugs will 
         remain.  (Should mostly only effect documents that used
         \noist with a custom Xindy style file.)

   * \printglossary sets \currentglossary to the current glossary's
     label. (Allows custom glossary styles access to the glossary
     type.)

   * Modified internal workings of acronyms and:

     - Added starred versions of \acrshort etc.

     - Added "long", "short", "longplural" and "shortplural" keys
       (Reserved for use with \newacronym.)

     - Added analogous "longaccess", "shortaccess", "longpluralaccess"
       and "shortpluralaccess" keys for \newacronym in 
       glossaries-accsupp.sty

   * Added \glsseeitemformat to customise the text given in the link
     created by \glsseeitem.

   * \newglossaryentry key "nonumberlist" now boolean.

   * added debugging commands \showgloname etc.

   * now loads etoolbox:

     - replaced \DeclareRobustCommand with \newrobustcmd

     - replaced \@ifundefined with \ifcsundef

     - replaced \let...\undefined with \undef...

   * Bug Fixes:

     - now works with equation counter in amsmath's align
       environment.

     - Mixed counters now work with xindy option.

     - Fixed hyperlinks in location numbers where \theH<counter>
       has a prefix not present in \the<counter>.

     - If title specified in \printglossary but toctitle hasn't
       been specified, make toctitle same as supplied title.

     - \newglossaryentry "see" key and \glssee now sanitize and escape 
       special characters before writing to output file. (Allows
       user to redefine \seename any point before \printglossary or
       \printglossaries.)

     - \glshyperlink: Changed the default value of the optional argument
                      to \glsentrytext instead of \glsentryname.

   * mfirstuc.sty (v1.05):

     - added \glsmakefirstuc (replaces \@gls@makefirstuc) to make
       it easier to customise.

   makeglossaries (v2.02):

   * now displays version number on startup unless -q

   * added more diagnostics to give more helpful messages than
     those supplied by xindy or makeindex.

v2.07:

   * Fixed bug that ignored format key in \glsadd

   makeglossaries:

   * Fixed bug causing failure to process aux files containing \@input

v2.06:
   * Added \altnewglossary

   * added facility to customise acronyms if the predefined styles
     don't fit the user's requirements.

   * Serbian dictionary added (provided by Zoran Filipovic)

   makeglossaries:

   * Scans aux file for \@input in case \printglossary is in an
     imported file.

v2.05:
   * Fixed error in .ist file and in \glsdisp caused by a 
     misplace brace. (Patch provided by Sergiu Dotenco).

v2.04:
   * Improved support for multiple lists of acronyms.

   * Fixed bug that caused \glsadd to ignore counter option

   * Fixed bug that causes babel to override translator's definition
     of \glossaryname.

   * Added user1, ... , user6 keys.

   * Added polyglossia support

   * makeglossaries now creates stub output file if input file is
     empty

  glossaries-accsupp v0.2:
   * Added access keys.

   * Added support for acronyms.

  mfirstuc v1.04: 
   * fixed bug occurring when initial control sequence
     in the argument of \makefirstuc has more than one 
     argument.

v2.03:
   * Added check to see if \glossarymark has been defined

   * makeglossaries - failed file test messages printed to
     stdout instead of stderr (so that it doesn't interrupt
     latexmk).

   * Fixed bug when entries used at the start of a paragraph.

   * Added package option hyperfirst (boolean option to suppress
     hyperlink on first use).

   * Added pod to makeglossaries.

v2.02:
   * Renamed glossaries-dictionary-Brazil.dict to 
     glossaries-dictionary-Brazilian.dict

   * Replaced \@mkboth with \glossarymark in \glossarysection
     to make it easier for the user to override it

   * Fixed bug that generated no \printglossary warning when
     the glossary is placed in a group

   * translate=false option will now prevent automatic loading
     of translator package.

v2.01:
   * Documentation changes:
      - removed quick guide section from glossaries.pdf and replaced 
        it with a separate beginners guide (glossariesbegin.pdf)
      - added a section for front-end or script developers who
        want to access information from the aux file

   * Added new ragged right versions of long/super styles

   * Added 'nomain' package option to suppress the creation of the
     main glossary

   * Added 'nowarn' package option to suppress warnings

   * Removed unwanted full stops in transcript messages

   * Changed \linewidth to \hsize when setting lengths

   * Removed item_02 key from makeindex style file (no such key)

   * Moved \@do@wrglossary before term is displayed to prevent
     unwanted whatsit

v2.0 (1.20):
   * Fixed ngerman caption bug in glossaries-babel.sty

v1.19:

   * changed \acronymfont to use \textsmaller instead of \smaller
     (for "smaller" package option)

   * Added \glsdisp (similar to \glslink except that it uses
     \glsdisplay/glsdisplayfirst and unsets the first use flag)

   * Added experimental package glossaries-accsupp which 
     requires accsupp package.

v1.18:
   * fixed missing closing } in glossaries-babel.sty

   * added \glstarget so that glossary styles can be modified
     in the document without using internal commands.

   * glossary-super.sty isn't loaded if supertabular.sty isn't
     installed.

   * added nolong, nosuper, nolist, notree and nostyles package 
     options to prevent loading unnecessary packages.

   * added \oldacronym (emulates the old glossary package's 
     \newacronym command).

   * added sublistdotted style.

   * fixed bug caused by misspelt \glspagewidthlist (should be
     \glspagelistwidth).

   * fixed border in super4colheaderborder and 
     altsuper4colheaderborder styles.

   * fixed sort sanitization when package option sanitize={name=false}
     is used.

v1.17:
   * changed definition of \@glossary to prevent conflict with
     memoir

   * added check to determine if \printglossary is defined. (If
     it is, issue warning and redefine.)

   * provided means to suppress number list for specific entries

   * provided means to suppress description terminator for
     specific entries

   * added cross-referencing support

   * added hierarchical support

   * added xindy support

   * modified \glshypernumber to support \nohyperpage
     (code provided by Heiko Oberdiek)

   * added 2 and 3-page suffix support

   * added "order" package option to set word/letter ordering
     (only has an effect in combination with makeglossaries script)

   * added Brazilian dictionary (supplied by Thiago de Melo)

v1.16 :
   * fixed bug that causes footnote option to remove hyperlink
     for first use entries in glossaries other than the list
     of acronyms. (footnote option should only affect entries
     in \acronymtype glossary.)

   * Raised hypertarget so that links to glossary entries don't
     scroll off the top of the page.

   * Fixed expansion-related bug (thanks to fix provided by
     Ulrich Diez)

v1.15 :
   * added \glslabel

   * added altlong4col* and altsuper4col* styles

   * fixed PDF encoding problem caused when both translator
     and hyperref packages are being used

   * fixed bug when using smallcaps and smaller options that causes
     the long form in the list of acronyms to be the same for each 
     entry

   * Added warnings when rerun required when using glossary
     group hyper navigation

glossaries.perl v1.04:
   * add do_cmd_glslabel

   * changed links to the start of the relevant glossary entry
     rather than the entry's backlink

   * added implementation of starred forms of \gls etc

   * added frame related code if frames.pl has been loaded

v1.14 :
   * Fixed bug in \glsnavhyperlink that causes an error when used
     with hyperref and translator packages.

   * Added \glsautoprefix (specifies a prefix to the automatically
     generated label)

   * Added nonumberlist and numberedsection keys to \printglossary

   * Changed \glsnavigation so that it only lists the groups that
     are present. (This prevents unknown target warnings.)

   * Amended documentation.

mfirstuc v1.02 (18 June 2008):

   * Fixed bug that transfered grouping, (e.g 
     \makefirstuc{\emph{abc}xyz} moved the xyz into the \emph)

   * If group following initial command is empty, \MakeUppercase
     is applied to the command, e.g. \makefirstuc{\ae{}bc} now
     produces \MakeUppercase\ae{}bc.

v1.13 :
   * Fixed bug in long4colheaderborder that puts an extra row
     at the end of the glossary.

   * Fixed bug in \glstext etc that ignored 3rd argument (thanks
     to Franz Fischer for pointing this out).

   * Removed only preamble restriction on \newglossaryentry and
     \newacronym.

   * Added \glspluralsuffix.

   * Changed firstplural default so that it takes its value from
     the plural key if the first key is omitted.

   * Added \acrshortpl, \Acrshortpl, \ACRshortpl, \acrlongpl,
     \Acrlongpl, \ACRlongpl, \acrfullpl, \Acrfullpl, \ACRfullpl.

   * Fixed bugs in \Acrshort etc.

   * Add package options "smaller" and "shortcuts".

   * Acronym default plural forms now implemented for the additional
     acronym styles.

   * Fixed makeglossaries to allow filenames with spaces.

   * Fixed error in documentation describing \glsaddall
     - optional argument should be a key=value list.

   * Added Polish support (thanks to Piotr Formella for supplying
     the translations).

   * If babel is loaded and translator package is found on TeX's
     path, then the translator package will now be automatically 
     loaded.

mfirstuc v1.01 (13 May 2008):

   * Added \xmakefirstuc (expands argument before applying \makefirstuc)

v1.12 (8 March 2008):
   * Fixed bug that causes \glspl to print the plural short form
     on first use instead of the plural long form.

   * Added descriptionplural and symbolplural keys.

   * Added \glsshortkey, \glsshortpluralkey, \glslongkey and
     \glslongpluralkey.

   * Fixed bugs in \glsname, \glstext, \glsdesc etc.

   * Added a check for \hypertarget in addition to checking
     for \hyperlink (in the event that \hyperlink is defined
     but not \hypertarget).

   * Changed #! line in makeglossaries to use /usr/bin/env

   * Added package mfirstuc.sty which provides the command 
     \makefirstuc{<stuff>} which makes the first object of
     <stuff> uppercase unless <stuff> starts with a control
     sequence followed by a group, in which case the first
     object in the group is converted to uppercase. Examples:

     \makefirstuc{abc}        -> Abc
     \makefirstuc{\emph{abc}} -> \emph{Abc}
     \makefirstuc{{\'a}bc}    -> {\'A}bc
     \makefirstuc{\ae bc}     -> \AE bc
     \makefirstuc{{\ae}bc}    -> {\AE}bc

     (but don't do \makefirstuc{\ae{}bc} which produces \ae Bc.)

v1.11 (2 March 2008):
   * Fixed error in manual (glossary style is set using \glossarystyle
     not \setglossarystyle).

   * Changed the way the package is archived to make it compatible
     with TeX Live.

   * Improved error handling of makeglossaries and added --version
     and --help options.

v1.1 (22 Feb 2008):

   * New package options:

     - numberline: 
       inserts \numberline{} in \addcontentsline when used with
       the toc option.

     - numberedsection: 
       puts glossaries in numbered chapters/sections

     - translate:
       translate=false option prevents glossaries package from
       using pre-supplied translations.

     - description:
       changes definition of \newacronym to allow a description

     - footnote:
       changes definition of \newacronym to use a footnote on
       first use

     - smallcaps:
       changes definition of \newacronym to set acronyms in 
       small capitals

     - dua:
       changes definition of \newacronym to always expand
       acronyms

   * Added \setglossarysection
     - changes the section type used by the glossaries

   * Added listdotted glossary style.

   * No longer uses xspace package; uses amsgen instead.

   * Added \glsname, \glsdesc, \glssymbol, \glsfirst, \glstext, 
     \glsplural and \glsfirstplural.

   * Added support for translator package.

v1.08 (13 Oct 2007):
   * Added multilingual support
   * Fixed bug in listgroup and altlistgroup styles so that 
     \glsgroupheading uses \glsgetgrouptitle to get the group title 
     instead of displaying the label
   * Fixed typo in error message text when the description key
     is missing to \newglossaryentry.

v1.07 (13 Sep 2007):
   * Fixed bug causing incorrect page number for entries in the
     first paragraph of a page.

v1.06 (21 Aug 2007):
   * Changed the license text

v1.05 (10 Aug 2007):
   * Changed the default value of the sort key to just use the
     name key
   * Added \@mkboth to \glossarysection

v1.04 (3 Aug 2007):
   * Added \glstextformat

v1.03 (4 July 2007):
   * Added \glspostdescription

v1.02 (25 May 2007):
   * Added overview section in the documentation

v1.01 (17 May 2007):
   * Added number range facility (equivalent to makeindex's |( and |)
     formatting commands.)
   * Added a space after \delimN and \delimR in the ist file.

v1.0 (16 May 2007): Initial release


==> cmd-math.tex <==

%%%%%%%%%%%% COMMANDES DE MATHS %%%%%%%%%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{amsthm} % proof, etc.

\newcommand{\R}{\mathbb{R}} 			% |R
\newcommand{\Z}{\mathbb{Z}} 			% Z
\newcommand{\N}{\mathbb{N}} 			% |N

\newcommand{\LL}{{\mathcal L}} 			% Lattice


\newcommand{\PPE}{\leqslant}  			% < =
\newcommand{\PGE}{\geqslant}   			% > =
\newcommand{\IFF}{\Longleftrightarrow}  	% <-->
\newcommand{\Fleche}{\Rightarrow}		% -->
\newcommand{\fleche}{\rightarrow}		% ->	
\newcommand{\takes}{\leftarrow}			% <-
\newcommand{\PartsOf}[1]{{\cal P}({#1})}	% P(X) partie d'un ensemble
%\newcommand{\LimN }{ \lim_{n \to \infty} }	% lim n -> +inf
\newcommand{\LimInf }[1]{ \lim_{#1 \to \infty} } % lim ? -> +inf
\newcommand{\eq}{\thicksim}			% ~
%\newcommand{\implies}{\RightArrow}		% =>
\newcommand{\function}[3]{ {#1} : {#2} \fleche  {#3} } 	% f: X -> Y

\newcommand{\forallin}[2]{{\forall #1 \in #2, \, \, }}


%% probas
\newcommand{\Prob}[1]{\Pr\set{#1}}
\newcommand{\Exp}[1]{\mathbb{E}\set{#1}}
\newcommand{\var}[1]{\mathrm{var}\Braces{#1}}

\newcommand{\wproba}{\text{ with probability }}
\newcommand{\Ber}{\mathcal{B}}                  % Bernoulli
\newcommand{\fInd}[3]{\mathcal{#1}_{#3,#2}}     % Bernoulli-like


% intervals
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Interval}[2]{\set{{#1},\dots,{#2}}}
\newcommand{\OneTo}[1]{\set{1,\dots,{#1}}}

%%% typesetting

\newcommand{\und}[1]{_{\mathrm{#1}}}

%%%%% operators
\newcommand{\SuchThat}{{\, | \,}} % first version
%\newcommand{\SuchThat}{{\, , \,}} % other version

\newcommand{\et}{\mbox{ et }}
\newcommand{\si}{\mbox{ si }}
\newcommand{\ou}{\mbox{ ou }}
\newcommand{\TextAnd}{\mbox{ and }}
\newcommand{\TextIf}{\mbox{ if }}
\newcommand{\TextOr}{\mbox{ or }}
\newcommand{\TextOtherwise}{\mbox{ otherwise }}


\newcommand{\TextEt}{\mbox{ et }}
\newcommand{\TextSi}{\mbox{ si }}
\newcommand{\TextOu}{\mbox{ ou }}
\newcommand{\TextSinon}{\mbox{ sinon }}

%scientific notation
\newcommand{\ten}[1]{{\ensuremath{10^{#1}}}}
\newcommand{\sn}[2]{{\ensuremath{#1 \times 10^{#2}}}}
\newcommand{\thousand}{\, 000}

\newcommand{\SqBrackets}[1]{\big[\, #1 \,\big]}
\newcommand{\Brackets}[1]{\big(\, #1 \,\big)}
\newcommand{\Braces}[1]{\big\{\, #1 \,\big\}}

\newcommand{\Sum}[2]{\sum_{#1}^{#2}}


==> makeglossaries <==
#!/usr/bin/env perl

# File    : makeglossaries
# Author  : Nicola Talbot
# Version : 4.41
# Description: simple Perl script that calls makeindex or xindy.
# Intended for use with "glossaries.sty" (saves having to remember
# all the various switches)

# This file is distributed as part of the glossaries LaTeX package.
# Copyright 2007 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

# This work consists of the files glossaries.dtx and glossaries.ins 
# and the derived files glossaries.sty, glossaries-prefix.sty,
# glossary-hypernav.sty, glossary-inline.sty, glossary-list.sty, 
# glossary-long.sty, glossary-longbooktabs.sty, glossary-longragged.sty,
# glossary-mcols.sty, glossary-super.sty, glossary-superragged.sty, 
# glossary-tree.sty, glossaries-compatible-207.sty, 
# glossaries-compatible-307.sty, glossaries-accsupp.sty, 
# glossaries-babel.sty, glossaries-polyglossia.sty, glossaries.perl.
# Also makeglossaries and makeglossaries-lite.lua.

my $version="4.41 (2018-07-23)";

# History:
# v4.41:
#   * No change.
# v4.40:
#   * No change.
# v4.39:
#   * No change.
# v4.38:
#   * No change.
# v4.37:
#   * No change.
# v4.36:
#   * No change.
# v4.35:
#   * No change.
# v4.34:
#   * Added check for \glsxtr@resource
# v4.33:
#   * Version number synchronized with glossaries.sty
# v2.21:
#   * Fixed spelling of \GlsAddXdyLocation
#   * Adjusted range encap clash
# v2.20 (2016/12/16)
#   * Added check for \glsxtr@makeglossaries
# v2.19 (2016/05/27)
#   * Improved check in &parse_for_xindy_nosort
# v2.18 (2016/01/24)
#   * Added &parse_for_xindy_nosort to help diagnose xindy's empty
#     index key warning/error.
#   * Added check for makeindex's multiple encap warning.
# v2.17 (2015/11/30)
#   * Escaped { in regular expressions.
#     http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=101
# v2.16 (2015/06/28)
#   * Added check for "german" and codepage that doesn't contain
#   "din5007", "duden" or "braille". If missing, "din5007-" is
#   prefixed to the codepage.
# v2.15 (2014/07/30)
#   * Removed hard-coded three character extension assumption
#     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=55
#   * Added message to indicate the number of ignored glossaries
#     when the extension is specified.
# v2.14 (2014/03/06)
#   * Added -Q and -k options
# v2.13 (2014/01/21)
#   * Added check for leading and trailing quotes in filename
# v2.12 (2014/01/20)
#   * Added check for '*' in istfilename
#   * Fixed bug report
#   http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=33
#   * Added error text hashes
# v2.11 (2014/01/17):
#   * Added check for backslashes in -x, -m and -d paths
#   * Added double-quotes around $appname in &run_app
# v2.10 (2013/12/01):
#   * initialise $language to suppress warnings
# v2.09 (2013-11-12):
#   * added check for -q switch when issuing warnings.
# v2.08 (2013-10-14):
#   * added -x and -m options
# v2.07 (2013-06-17):
#   * added check for success on chdir if -d used
#   * added dialect map
# v2.06 (2013-04-21):
#   * added "din5007" as default if language is set to "german"
# v2.05 (2012-11-12):
#   * added -d option
# v2.04 (2012-04-19):
#   * fixed bug in &scan_aux
# v2.03 (2011-04-12):
#   * added warning about possibly needing 'nomain' package option
# v2.02 (2011-04-2):
#   * Prints version number at start of run unless -q
#   * Added more diagnostics.
# v2.01 (2010-09-29):
#   * Added 'use warnings'
# v2.0 (2010-06-30) :
#   * Made file handle local in &scan_aux
# v1.9 (2010-06-14) :
#   * Check for \@input
# v1.8 (2009-11-03) :
#   * Create an empty output file if the input file is empty
#     without calling xindy/makeindex
# v1.7 (2009-09-23) :
#   * Issue warning rather than error when empty/non existant file 
#     checks fail
# v1.6 (2009-05-24) :
#   * main glossary no longer automatically added
#     (only added if information in aux file)
#   * if file extension is specified, check added to ensure it
#     corresponds to a known glossary extension.
#   * added file existance test and file empty test
# v1.5 (2008-12-26) :
#   * added support for xindy
#   * picks up ordering information from aux file
# v1.4 (2008-05-10) :
#   * added support for filenames with spaces.
# v1.3 (2008-03-08) :
#   * changed first line from /usr/bin/perl -w to /usr/bin/env perl
#     (Thanks to Karl Berry for suggesting this.)
# v1.2 (2008-03-02) :
#   * added support for --help and --version
#   * improved error handling
# v1.1 (2008-02-13) :
#   * added -w and strict
#   * added check to ensure .tex file not passed to makeglossaries
#
# v1.0 (2007-05-10) : Initial release.

use Getopt::Std;
use strict;
# v2.01 added the following line
use warnings;
# v2.05 added $opt_d
# v2.08 added $opt_x and $opt_m
use vars qw($opt_q $opt_t $opt_o $opt_s $opt_p $opt_g $opt_c $opt_r
   $opt_l $opt_i $opt_L $opt_n $opt_C $opt_d $opt_x $opt_m $opt_Q
   $opt_k);


$Getopt::Std::STANDARD_HELP_VERSION = 1;

# v1.5 added -L <lang> for xindy (but language can be specified in 
# .tex file)
# v1.5 added -n (print the command that would be issued but
# don't actually run the command)
getopts('s:o:t:p:L:C:ilqQkrcgnd:x:m:');

unless ($#ARGV == 0)
{
   die "makeglossaries: Need exactly one file argument.\n",
       "Use `makeglossaries --help' for help.\n";
}

# v2.02: added:
print "makeglossaries version $version\n" unless ($opt_q);

# v2.07: added babel dialect -> xindy language map:
my %languagemap =
(
  'american'  => 'english',
  'austrian'  => 'german',
  'british'   => 'english',
  'francais'  => 'french',
  'frenchb'   => 'french',
  'germanb'   => 'german',
  'lsorbian'  => 'lower-sorbian',
  'magyar'    => 'hungarian',
  'naustrian' => 'german',
  'ngermanb'  => 'german',
  'ngerman'   => 'german', # v2.16
  'norsk'     => 'norwegian',
  'portuges'  => 'portuguese',
  'russianb'  => 'russian',
  'slovene'   => 'slovenian',
  'UKenglish' => 'english',
  'USenglish' => 'english',
  'ukraineb'  => 'ukrainian',
  'usorbian'  => 'upper-sorbian'
);

# v2.07 added check for success and for -q
# v2.05 added:

if ($opt_d)
{
  # v2.11 check for backslash character if on Windows
  $opt_d=~s/\\/\//g if $^O=~/Win/;

  if (chdir $opt_d)
  {
     print "Changed to '$opt_d'\n" unless ($opt_q);
  }
  else
  {
     die "Unable to chdir to '$opt_d' $!\n";
  }
}

# v2.02: added:
# v2.19: changed value
my $xdynotist = 2;
# v2.13: removed
#my $needcompatibilitymode=2;

# v2.13: added $istnotfound
my $istnotfound = 3;

# v2.13: added error text:
my %makeindex_error_text =
 (
   $xdynotist => "Style name indicates makeindex, but may be in xindy format.\n"
          . "Remember to use \\setStyleFile to specify the name\n"
          . "of the style file rather than redefining \\istfilename\n"
          . "explicitly.",
   $istnotfound => "Style file not found. (Have you used \\noist by mistake?)"
 );

my %xindy_error_text =
 (
   'nosort'    => "Sort key required for entries only containing command names.",
   'istnotxdy' =>
      "Style name has xdy extension, but may be in makeindex format.\n"
     . "Remember to use \\setStyleFile to specify the name\n"
     . "of the style file rather than redefining \\istfilename\n"
     . "explicitly.",
   'missingendquote' =>
       "You may have missed a \" character in a command such as \\GlsAddXdyLocation.",
    'nolanguage' =>
       "No language detected.\nHave you remembered to use \\printglossary\n".
       "or \\printglossaries in your document?",
    'nomain' =>
        "\nRemember to use package option 'nomain' if you don't\n".
        "want to use the main glossary.",
#v2.21: fixed spelling of \GlsAddXdyLocation
    'badlocation' =>
        "You may have forgotten to add a location \n"
        . "class with \\GlsAddXdyLocation or you may have \n"
        . "the format incorrect.\n",
    'comp207' => "You may need to add 'compatible-2.07' package option.",
    'noxdyfile' => "Style file not found. (Have you used \\noist by mistake?)"
 );

# define known extensions

# v1.6: removed adding main glossary here as there's no guarantee
# that it's been used. If it has been used, the information will
# be picked up later in the aux file
my %exttype = (
#   main => {in=>'glo', out=>'gls', 'log'=>'glg'},
 );

# v1.5 define require languages for xindy

my %language = ();
my %codepage = ();

my $ext = '';
my $name = $ARGV[0];

# v2.13 added:
#$name=~s/^"(.*)"$/$1/;
# v2.15: fix provided by Herb Schulz to allow for extensions that
# aren't exactly three characters:
# (HS) changes fix for 3 character extension limit
my ($basename,$extension) = ($name =~ m/^(.*?)(?:\.([^\.]*))?$/);
# (HS) end of changes fix for 3 character extension limit

# make sure $extension is defined. (If there was no match in the
# above, it cause an uninitialised error later.)
$extension = '' unless ($extension);

# Make sure users don't try passing the tex file:

#if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
#{
#  $name = substr($ARGV[0],0,length($ARGV[0])-4);
#
#  $ext = substr($ARGV[0],-3,3);
#
#  if (lc($ext) eq 'tex')
# (HS) changes fix for 3 character extension limit
#if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
#{
#  $name = substr($ARGV[0],0,length($ARGV[0])-4);
#
#  $ext = substr($ARGV[0],-3,3);
#
#  if (lc($ext) eq 'tex')
  if (lc($extension) eq 'tex')
  {
     die("Don't pass the tex file to makeglossaries:\n"
        ."either omit the extension to make all the glossaries, "
        ."or specify one of the glossary files, e.g. $name.glo, to "
        ."make just that glossary.\n")
  }
#}
# (HS) end of fix for 3 character extension limit

# (HS) changes fix for 3 character extension limit
$ext = $extension;
$name = $basename;
# (HS) end of changes fix for 3 character extension limit

# v2.01 add check to see if aux file exists

unless (-e "$name.aux")
{
   die "Auxiliary file '$name.aux' doesn't exist. Have you run LaTeX?\n";
}

my $istfile = "";

my $glslist = "";

# should letter ordering be used? (v1.5 added)

my $letterordering = defined($opt_l);

# v2.19 added:
my $extramkidxopts = '';

# v4.34 added:
my $foundbib2glsresource = '';

# Check aux file for other glossary types,
# style file name and various other bits of information.

&scan_aux($name);

# has the style file been specified?
unless ($istfile)
{
   if ($foundbib2glsresource)
   {
      die "Found \\glsxtr\@resource in '$name.aux',\n",
          "but not found \\\@istfilename.\n",
          "You need to run bib2gls not makeglossaries.\n";
   }
   else
   {
      die "No \\\@istfilename found in '$name.aux'.\n",
          "Did your LaTeX run fail?\n",
          "Did your LaTeX run produce any output?\n",
          "Did you remember to use \\makeglossaries?\n";
   }
}

# v2.08 added $xindyapp and $makeindexapp
# By default assume they are on the operating system's path
my $xindyapp = ($opt_x ? $opt_x :'xindy');
my $makeindexapp = ($opt_m ? $opt_m :'makeindex');

# v2.11 check for backslash character if on Windows
if ($^O=~/Win/)
{
  $xindyapp=~s/\\/\//g;
  $makeindexapp=~s/\\/\//g;
}

# v1.5 save the general xindy switches

my $xdyopts = '';

# v2.01 replaced 'unless ($opt_L eq "")' with 'if ($opt_L)'
if ($opt_L)
{
  $xdyopts .= " -L $opt_L";
}

# save all the general makeindex switches

my $mkidxopts = '';

if ($opt_i)
{
   $mkidxopts .= " -i";
}

if ($letterordering)
{
   $mkidxopts .= " -l";
   $xdyopts .= " -M ord/letorder";
}

if ($opt_q)
{
# v2.01 removed following lines. (This script now deals with
# printing messages to STDOUT.)
   #$mkidxopts .= " -q";
   #$xdyopts .= " -q";
}

if ($opt_r)
{
   $mkidxopts .= " -r";
}

if ($opt_c)
{
   $mkidxopts .= " -c";
}

if ($opt_g)
{
   $mkidxopts .= " -g";
}

# v2.01 replaced 'unless ($opt_p eq "")' with 'if ($opt_p)'
if ($opt_p)
{
   $mkidxopts .= " -p $opt_p";
}

if ($extramkidxopts)
{
  $mkidxopts .= " $extramkidxopts";
}

# v2.01 replaced 'unless ($opt_s eq "")' with 'if ($opt_s)'
if ($opt_s)
{
   # v2.01 check if user has specified -s <file>.ist but aux file
   # indicates .xdy ought to be used and vice-versa. Also check if
   # requested style file exists

   unless (-e $opt_s)
   {
      die "\n",
         "Requested style file '$opt_s' doesn't exist.\n\n";
   }

   if ($istfile=~/\.xdy$/ and $opt_s!~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using xindy,\n",
        "but you have specified makeindex style file '$opt_s'\n",
        "Make sure you don't specify 'xindy' as a package option if\n",
        "you want to use makeindex.\n\n",
        "\\usepackage[makeindex]{glossaries}\n\n";
   }
   elsif ($istfile!~/\.xdy$/ and $opt_s=~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using\n",
        "makeindex, but you have specified xindy style file '$opt_s'.\n",
        "Make sure you specify 'xindy' as a package option if you\n",
        "want to use xindy.\n\n",
        "\\usepackage[xindy]{glossaries}\n\n";
   }

   $istfile = $opt_s;
}

# Use xindy if style file ends with .xdy otherwise use makeindex

my $usexindy = ($istfile=~m/\.xdy\Z/);

if ($ext)
{
   # an extension has been specified, so only process
   # the specified file

   # v1.6 %thistype is no longer given a default value
   my %thistype;

   my $thislang = "";
   my $thiscodepage = "";

   my @types = ($glslist ? split /,/, $glslist : keys %exttype);

   foreach my $type (@types)
   {
      if ($exttype{$type}{'in'} eq $ext)
      {
         %thistype = %{$exttype{$type}};

         $thislang = $language{$type};

         $thiscodepage = $codepage{$type};

         last;
      }
   }

   # v1.6 If %thistype hasn't been defined, then the given
   # extension doesn't correspond to any known glossary type

   # v2.01 replaced deprecated 'defined(%thistype)' with %thistype
   unless (%thistype)
   {
      die "The file extension '$ext' doesn't correspond to any\n",
          "known glossary extension. Try running makeglossaries\n",
          "without an extension, e.g. makeglossaries \"$name\".\n";
   }

   my $outfile;

# v2.01 replaced 'if ($opt_o eq "")' with 'unless ($opt_o)'
   unless ($opt_o)
   {
      $outfile = "$name.$thistype{out}";
   }
   else
   {
      $outfile = $opt_o;
   }

   my $transcript;

# v2.01 replaced 'if ($opt_t eq "")' with 'unless ($opt_t)'
   unless ($opt_t)
   {
      $transcript = "$name.$thistype{'log'}";
   }
   else
   {
      $transcript = $opt_t;
   }

# v2.01 remove old transcript file

   unless ($opt_n)
   {
      unlink($transcript);
   }

   if ($usexindy)
   {
      &xindy("$name.$ext", $outfile, $transcript,$istfile,
        $thislang, $thiscodepage, $xdyopts, $opt_q, $opt_n, $xindyapp);
   }
   else
   {
      &makeindex("$name.$ext",$outfile,$transcript,$istfile,
                 $mkidxopts,$opt_q, $opt_n, $makeindexapp, 1);
   }


   # v2.15 added:

   my $num_omitted = $#types;

   if ($num_omitted == 1)
   {
      print "1 glossary ignored.\n" unless $opt_q;
   }
   elsif ($num_omitted > 1)
   {
      print "$num_omitted glossaries ignored.\n" unless $opt_q;
   }
}
else
{
   # no file extension specified so process all glossary types

   my @types = ($glslist ? split /,/, $glslist : keys %exttype);

   foreach my $type (@types)
   {
      my %thistype = %{$exttype{$type}};

      my $inputfile = "$name.$thistype{in}";

      my $outfile;

# v2.01 changed 'if ($opt_o eq "")' with 'unless ($opt_o)'
      unless ($opt_o)
      {
         $outfile = "$name.$thistype{out}";
      }
      else
      {
         $outfile = $opt_o;
      }

      # v1.7 print warnings to STDOUT instead of STDERR

      # v1.6 added file existence test
      unless (-e $inputfile)
      {
         # v2.09 suppress warning if -q switch in use
         print "Warning: File '$inputfile' doesn't exist.\n",
             "*** Skipping glossary '$type'. ***\n" unless ($opt_q);
         next;
      }

      unless (-r $inputfile)
      {
         print "Warning: No read access for '$inputfile' $!\n",
             "*** Skipping glossary '$type'. ***\n" unless ($opt_q);
         next;
      }

      my $transcript;

# v2.01 changed 'if ($opt_t eq "")' with 'unless ($opt)'
      unless ($opt_t)
      {
         $transcript = "$name.$thistype{'log'}";
      }
      else
      {
        $transcript = $opt_t;
      }

      # v1.6 added file empty test
      if (-z $inputfile)
      {
         my $message =
             "Warning: File '$inputfile' is empty.\n".
             "Have you used any entries defined in glossary '$type'?\n";

         if ($type eq 'main')
         {
            $message .=
               "Remember to use package option 'nomain' if you\n".
               "don't want to use the main glossary.\n";
         }

         # v2.09 suppress warning if -q switch in use
         warn $message unless $opt_q;

         # Write warning to transcript file.

         if (open TRANSFD, ">$transcript")
         {
            print TRANSFD $message;
            close TRANSFD;
         }

         # create an empty output file and move on to the next glossary

         if (open OFD, ">$outfile")
         {
            print OFD "\\null\n";
            close OFD;
         }
         else
         {
            warn "Unable to create '$outfile' $!\n";
         }

         next;
      }

# v2.01 remove old transcript file

      unless ($opt_n)
      {
         unlink($transcript);
      }

      if ($usexindy)
      {
         &xindy($inputfile,$outfile,$transcript,$istfile,
                $language{$type},$codepage{$type},
                $xdyopts,$opt_q,$opt_n, $xindyapp);
      }
      else
      {
         &makeindex($inputfile,$outfile,$transcript,
                    $istfile,$mkidxopts,$opt_q,$opt_n, $makeindexapp, 1);
      }
   }
}

sub scan_aux{
  my $name = shift;

  # v2.0 added
  local(*AUXFILE);

  if (open AUXFILE, "$name.aux")
  {
     while (<AUXFILE>)
     {
        #v2.14 added
        if (m/\\\@gls\@reference/ and not $glslist)
        {
           die "Your document has used \\makenoidxglossaries\n",
               "You don't need makeindex or xindy.\n";
        }

        if (m/\\glsxtr\@makeglossaries\{(.*)\}/)
        {
           #v2.20 added

           $glslist = $1;

           unless ($opt_q)
           {
              print "only processing subset '$glslist'\n";
           }
        }
        elsif (m/\\\@input\{(.+)\.aux\}/)
        {
           # v1.9 added
           # v2.17 escaped { in regex
           &scan_aux($1);

           # v2.04 added
           # (Fix provided by Daniel Grund) 
           next;
        }
        elsif (m/\\\@newglossary\s*\{(.*)\}\{(.*)\}\{(.*)\}\{(.*)\}/)
        {
           # v2.17 escaped { in regex

           $exttype{$1}{'log'} = $2;
           $exttype{$1}{'out'} = $3;
           $exttype{$1}{'in'}  = $4;

           unless ($opt_q)
           {
              print "added glossary type '$1' ($2,$3,$4)\n";
           }
        }
        elsif (m/\\\@istfilename\s*\{([^}]*)\}/)
        {
           # v2.17 escaped { in regex

           $istfile = $1;

           # check if double quotes were added to \jobname
           # v2.12 added check for xdy (bug ID 33)
           $istfile=~s/^"(.*)"\.(ist|xdy)$/$1.$2/;

           # v2.12 if on Windows, substitute any '*' with ' '
           # to compensate for MiKTeX bug
           # http://sourceforge.net/p/miktex/bugs/2301/

           if ($^O=~/Win/)
           {
              $istfile=~tr/\*/ /;
           }
        }
        elsif (m/\\\@xdylanguage\s*\{([^}]+)\}\{([^}]*)\}/)
        {
           # v1.5 added
           # v2.17 escaped { in regex

           $language{$1} = $2;
        }
        elsif (m/\\\@gls\@codepage\s*\{([^}]+)\}\{([^}]*)\}/)
        {
           # v1.5 added
           # v2.17 escaped { in regex

           $codepage{$1} = $2;
        }
        elsif (m/\\\@gls\@extramakeindexopts\{(.*)\}/)
        {
           # v2.19 added

           $extramkidxopts .= $1;
        }
        elsif (m/\\glsxtr\@resource/)
        {
           # v4.34 added

           # No error at this point as a hybrid method is allowed.
           # Error only occurs if no \@istfilename found.

           $foundbib2glsresource = 1;
        }

        # v1.5 added
        # Allow -l switch to override specification in aux file
        unless (defined($opt_l))
        {
           # v2.17 escaped { in regex
           if (m/\\\@glsorder\s*\{([^}]+)\}/)
           {
              my $ordering = $1;

              if ($ordering eq "word")
              {
                 $letterordering = 0;
              }
              elsif ($ordering eq "letter")
              {
                 $letterordering = 1;
              }
              else
              {
                 warn
                   "Unknown ordering '$ordering'\n",
                   "Assuming word ordering\n" unless ($opt_q);
                 $letterordering = 0;
              }
           }
        }
     }

     close AUXFILE;
  }
  else
  {
     warn "Unable to open $name.aux: $!\n";
  }
}

# v2.01 new subroutine run_app added
sub run_app{
   my($appname, $appargs, $trans, $quiet, $dontexec) = @_;

   local(*STATUS);

   my $status   = '';
   my $warnings = '';
   my $errno = 0;
   my $log = '';

   print "$appname $appargs\n" if ($dontexec or not $quiet);

   return if ($dontexec);

   # v2.11 added double-quotes around $appname
   # v2.14 added -k switch
   if (not $opt_k and open (STATUS, "\"$appname\" $appargs 2>&1 |"))
   {
      while (<STATUS>)
      {
         print unless ($quiet);

         $warnings .= $_ if (/WARNING:/);

         $status .= $_ unless (/^[\w]+ing/ or /^Finished/ or /^Usage:/);

         $log .= $_;
      }

      close STATUS;
   }
   else
   {
      unless ($opt_k)
      {
         $warnings = "Unable to fork \"$appname\" with redirection $!\n";

         # v2.14 added check for quiet switches
         warn $warnings,  
           "Retrying without redirection.\n" unless ($quiet or $opt_Q);
      }

      $status = `\"$appname\" $appargs`;

      $log = $status;

      print $status unless ($quiet);
   }

   if ($?)
   {
      # v2.14 Fixed error number assignment
      $errno = ($? >> 8);

      # v2.14 Added check for existence of transcript
      unless (-e $trans)
      {
         $log .= "\n$appname didn't create a transcript.\n";

         if (not $appname=~/\//)
         {
            # No path specified
            $log .= "Check that $appname has been installed and\nis on your system's PATH.\n";

            if (defined $ENV{PATH})
            {
               $log .= "Your PATH environment variable is set to: \n"
                    . $ENV{PATH} . "\n";
            }
            else
            {
               $log .= "I'm sorry, I can't detect your PATH environment variable\n";
            }

            $log .= "Try manually running:\n\"$appname\" $appargs\n";
         }
         elsif (not -e $appname)
         {
            if ($^O=~/Win/)
            {
               if (-e "$appname.exe" or -e "$appname.bat")
               {
                  $log .= "Try manually running:\n\"$appname\" $appargs\n";
               }
               else
               {
                  $log .= "File '$appname' doesn't exist.\n";
               }
            }
            else
            {
               $log .= "File '$appname' doesn't exist.\n";
            }
         }
         else
         {
            $log .= "Try manually running:\n\"$appname\" $appargs\n";
         }
      }

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n\n*** Unable to execute: '\"$appname\" $appargs' ***\n\n";
         print LOGFILE "Failed with error code $errno.\n\n";

         if ($log)
         {
            print LOGFILE "Status report:\n\n";
            print LOGFILE "$log", "\n";
         }

         print LOGFILE "Warnings:\n\n",$warnings, "\n" if $warnings;
         close LOGFILE;
      }
      else
      {
         warn "Unable to open '$trans' $!\n";
      }
   }

   if ($log=~/\(0 entries accepted,/
    or ( ($log=~/(\d+) warnings?/ and $1 gt 0))
    or $log=~/not found/)
   {
      # Attempt to diagnose what's gone wrong

      if (open TRANS, $trans)
      {
         while (<TRANS>)
         {
            if (/Index style file .* not found/)
            {
               $errno = $istnotfound;
               last;
            }
            elsif (/Unknown specifier ;/)
            {
               $errno = $xdynotist;
               last;
            }
            elsif (/## Warning \(.*\):\s*$/)
            {
               $warnings .= $_ . <TRANS>;
            }
         }

         close TRANS;
      }

   }

   return ($status, $warnings, $errno);
}

# v2.08 added $app parameter
sub makeindex{
   my($in,$out,$trans,$ist,$rest,$quiet,$dontexec,$app,$repairencaps) = @_;

   my $args = "$rest -s \"$ist\" -t \"$trans\" -o \"$out\" \"$in\"";

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app($app, $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($errno)
   {
      my $diagnostic = '';

      if ($makeindex_error_text{$errno})
      {
         $diagnostic = $makeindex_error_text{$errno};
      }
      else
      {
         $diagnostic = "Can't find diagnostic message for error code $errno";
      }

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\nmakeglossaries diagnostic messages:\n$diagnostic\n";
         close LOGFILE;
      }

      die "\n***Call to makeindex failed***\n", 
        ($diagnostic ?
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"
        ),
        "Check '$trans' for details\n";
   }

   # 2.18: added check and repair for multiple encaps
   if ($warnings)
   {
      warn $warnings unless $quiet;

      if ($repairencaps and $warnings=~/multiple encaps/)
      {
         unless ($quiet)
         {
            print "Multiple encaps detected. Attempting to remedy.\n";
            print "Reading $in...\n";
         }

         # if $in can't be opened at this point something wrong
         # has occurred (otherwise how did makeindex manage to open
         # it?)

         open INFD, $in or die "Can't open '$in' $!\n";

         my @entries = ();

         while (<INFD>)
         {
            if (/\\glossaryentry\{(.*)\|([^\|]*)\}\{(.*?)\}/)
            {
               my %entry = 
                (
                   'entry' => $1,
                   'encap' => $2,
                   'location' => $3
                );

               my $add = 1;

               for (my $idx = 0; $idx <= $#entries; $idx++)
               {
                  my $existing = $entries[$idx];

                  if ($entry{'entry'} eq $existing->{'entry'}
                  and $entry{'location'} eq $existing->{'location'}
                  and $entry{'encap'} ne $existing->{'encap'})
                  {
                     $add = 0 if ($add == 1);

                     # Range encaps should take precedence.

                     if ($entry{'encap'}=~/^[\(\)]/)
                     {
                        $add = 2;

                        if ($existing->{'encap'}=~/^[\(\)]/)
                        {
                           # too complicated, keep both

                           last;
                        }
                        else
                        {
                           # remove existing

                           splice @entries, $idx, 1;

                           $idx--;
                        }
                     }
                     elsif ($existing->{'encap'}=~/^[\(\)]/)
                     {
                        if ($entry{'encap'}=~/^[\(\)]/)
                        {
                           # too complicated, keep both

                           $add = 1;
                           last;
                        }
                        # (otherwise drop new entry)
                     }
                     elsif (&encap_overrides($entry{'encap'},
                                   $existing->{'encap'}))
                     {
                        $entries[$idx] = \%entry;
                     }
                  } 
               }

               push @entries, \%entry if $add > 0;
            }
            else
            {
               warn "Abandoning attempt. Can't parse: $_" unless $quiet;

               close INFD;
               return;
            }
         }

         close INFD;

         if (open OUTFD, ">$in")
         {
            print "Writing $in...\n" unless $quiet;

            foreach my $entry (@entries)
            {
               print OUTFD '\\glossaryentry{',
                 $entry->{'entry'}, '|',
                 $entry->{'encap'}, '}{',
                 $entry->{'location'}, '}', "\n";
            }

            close OUTFD;

            print "Retrying\n" unless $quiet;

            &makeindex($in,$out,$trans,$ist,$rest,$quiet,$dontexec,$app,0);
         }
         else
         {
            warn "Can't open '$in' $!\n" unless $quiet;
         }
      }
   }
}

# 2.18 new
# This is a subroutine in case of possible extension.
# For example, what happens in the event of 'textbf' and 'emph'?
# Should one override the other or be combined? Combining is harder
# as it would need a corresponding LaTeX command.
# 2.21 check for range encap moved earlier

sub encap_overrides{
  my ($newencap, $existing) = @_;

  ($existing=~/\\glsnumberformat\s*$/ or $newencap!~/\\glsnumberformat\s*$/ )
}

# v2.08 added $app parameter
sub xindy{
   my($in,$out,$trans,$ist,$language,$codepage,$rest,$quiet,
     $dontexec, $app) = @_;
   my($args, $langparam, $main, $retry);
   my($module);

   $module = $ist;
   $module=~s/\.xdy\Z//;

   if ($language)
   {
     # map babel names to xindy names

     $language = $languagemap{$language} if ($languagemap{$language});

     $langparam = "-L $language";
   }
   else
   {
     $langparam = "";
     # v2.10 initialise $language to suppress warnings
     $language = "";
   }

   # most languages work with xindy's default codepage, but
   # some don't, so if the codepage isn't specific, check
   # the known cases that will generate an error
   # and supply a default. (For all other cases, it's up to the 
   # user to supply a codepage.)

# v2.01 changed 'if ($codepage eq "")' to 'unless ($codepage)'
   unless ($codepage)
   {
      if ($language eq 'dutch')
      {
         $codepage = "ij-as-ij";
      }
      elsif ($language eq 'german')
      {
         $codepage = "din5007";
      }
      elsif ($language eq 'gypsy')
      {
         $codepage = "northrussian";
      }
      elsif ($language eq 'hausa')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'klingon')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'latin')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'mongolian')
      {
         $codepage = "cyrillic";
      }
      elsif ($language eq 'slovak')
      {
         $codepage = "small";
      }
      elsif ($language eq 'spanish')
      {
         $codepage = "modern";
      }
      elsif ($language eq 'vietnamese')
      {
         $codepage = "utf";
      }
   }
   elsif ($language eq 'german' and $codepage!~/(din5007|duden|braille)/)
   {
#v2.16 added check for german din/duden

      $codepage = "din5007-$codepage";
   }


   my $codepageparam = "";

   if ($codepage)
   {
      $codepageparam = "-C $codepage";
   }

   $main = join(' ',
      "-I xindy",
      "-M \"$module\"",
      "-t \"$trans\"",
      "-o \"$out\"",
      "\"$in\"");

   $args = join(' ', $rest, $langparam, $codepageparam, $main);

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app($app, $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($status=~/Cannot locate xindy module for language ([^\s]+) in codepage ([^\s]+)/)
   {
      $args = join(' ', $rest, $langparam, $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying using default codepage.\n";

         warn $message;

         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($status=~/Cannot locate xindy module for language ([^\s]+)/
    and $1 ne 'general')
   {
      $args = join(' ', $rest, "-L general", $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying with -L general\n";

         warn $message;
         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($errno)
   {
      # attempt further diagnostic

      my $diagnostic = '';

      if ($status=~/index 0 should be less than the length of the string/m)
      {
         $diagnostic = $xindy_error_text{nosort};

         $diagnostic .= &parse_for_xindy_nosort($in);
      }
      elsif ($status=~/variable .+ has no value/m)
      {
         # v2.19 fixed misspelt key
         $diagnostic = $xindy_error_text{istnotxdy};
      }
      elsif ($status=~/Could not find file /m)
      {
         # v2.19 added
         $diagnostic = $xindy_error_text{noxdyfile};
      }
      elsif ($status=~/Possible read-error due to ill-formed string " :sep/m)
      {
         $diagnostic = $xindy_error_text{missingendquote};
      }
      elsif (not $language)
      {
         # If the language hasn't been set, then it may be
         # because the document doesn't contain
         # \printglossaries/\printglossary or it may be
         # because the user has a customized style file that
         # contains the language settings.

          $diagnostic = $xindy_error_text{nolanguage};

          if ($in eq 'glo')
          {
             # or it may be that the user doesn't want to use the main
             # glossary and has forgotten to suppress it with the
             # "nomain" package option

             $diagnostic .= $xindy_error_text{nomain};
          }
      }

      # v2.19 added:
      if ($diagnostic and open LOGFILE, ">>$trans")
      {
         print LOGFILE "\nmakeglossaries diagnostic messages:\n\n$diagnostic\n";
         close LOGFILE;
      }

      die "\n***Call to xindy failed***\n", 
          ($diagnostic ? 
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"),
          "Check '$trans' for details\n";
   }

   # Check xindy warnings

   if ($status=~/^WARNING:/m)
   {
      my $diagwarn = '';

      if ($status=~/did not match any location-class/m)
      {
         $diagwarn = $xindy_error_text{badlocation};
      }

      if ($status=~/unknown attribute `pageglsnumberformat'/m)
      {
         $diagwarn .= $xindy_error_text{comp207};
      }

      if ($status=~/Would replace complete index key by empty string, ignoring/m)
      {
         $diagwarn .= $xindy_error_text{nosort};
         $diagwarn .= &parse_for_xindy_nosort($in);
      }

      if ($diagwarn)
      {
         warn "\n**Warning:**\n\n", $diagwarn, "\n";

         $warnings .= "\nmakeglossaries diagnostic messages:\n\n"
                   . $diagwarn;
      }
   }

   if ($retry or $warnings)
   {
      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n$warnings";

         if ($retry)
         {
            print LOGFILE "\nmakeglossaries messages:\n\n", $retry;
         }

         close LOGFILE;
      }
      else
      {
         warn "Unable to open '$trans' $!\n";
      }
   }
}

# v2.18 added:
sub parse_for_xindy_nosort{
  my ($in) = @_;

  my $msg = join("\n", "", 
                 "Attempting to determine which entries have problem sort keys.",
                 "Parsing '$in'");

  my %entries = ();

  if (open FD, $in)
  {
     while (<FD>)
     {
# v2.19 extra conditions added
        if (/:tkey \(\("((?:\\\\[a-zA-Z@]+ *)+)" "\\\\glossentry\{(.*)\}"\) \)/)
        {
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $label;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/([\\\s]+)//g;

           }
        }
        elsif (/:tkey \(\("(\\\\[a-zA-Z@]+ *{(?:\\\\[a-zA-Z@]+ *)+})+" "\\\\glossentry\{(.*)\}"\) \)/)
        {
# name in the form \cs{\cs}
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $1;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/^[a-zA-Z]+[:\-\.]//;
              $entries{$label}->{suggestion}=~s/([^\w]+)//g;
           }
        }
        elsif (/:tkey \(\("(\$\s*(?:\{?\\\\[a-zA-Z@]+ *\}?)+\$)" "\\\\glossentry\{(.*)\}"\) \)/)
        {
# name in the form $\cs$
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $1;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/^[a-zA-Z]+[:\-\.]//;
              $entries{$label}->{suggestion}=~s/([^\w]+)//g;
           }
        }
     }

     close FD;

     my @labels = keys %entries;

     my $n = $#labels+1;

     if ($n == 0)
     {
        $msg .= "\nCouldn't find anything! Sorry, I'm stumped.";
     }
     else
     {
        $msg .= ($n == 1 ? "\n1 problematic entry found:\n"
                         : "\n$n problematic entries found:\n");

        foreach my $label (@labels)
        {
           my $thisentry = $entries{$label};

           $msg .= "\nLabel: '$label'. Sort value : '$thisentry->{sort}'";
           $msg .= "\n(Try adding sort={$thisentry->{suggestion}} to the definition.)";
        }
     }
  }
  else
  {
     $msg .= "\nFailed to open '$in' $!\n";
  }

  $msg;
}

sub HELP_MESSAGE{
   print "\nSyntax : makeglossaries [options] <filename>\n\n";
   print "For use with the glossaries package to pass relevant\n";
   print "files to makeindex or xindy.\n\n";
   print "<filename>\tBase name of glossary file(s). This should\n";
   print "\t\tbe the name of your main LaTeX document without any\n";
   print "\t\textension.\n";
   print "\nGeneral Options:\n\n";
   print "-o <gls>\tUse <gls> as the output file.\n";
   print "\t\t(Don't use -o if you have more than one glossary.)\n";
   print "-q\t\tQuiet mode.\n";
   print "-Q\t\tSilence unable to fork warning.\n";
   print "-k\t\tDon't try to use piped redirection.\n";
   print "-l\t\tLetter ordering.\n";   
   print "-s <sty>\tEmploy <sty> as the style file.\n";
   print "-t <log>\tEmploy <log> as the transcript file.\n";
   print "\t\t(Don't use -t if you have more than one glossary\n";
   print "\t\tor the transcripts will be overwritten.)\n";
   print "-d <directory>\tDirectory in which the .aux, .glo etc files are located.\n",
     "\t\t(Default is the directory in which <filename> resides.)\n";
   print "-n\t\tPrint the command that would normally be executed,\n",
         "\t\tbut don't execute it.\n";

   print "\nXindy Options:\n\n";
   print "-L <language>\tUse <language>.\n";
   print "-x <file>\tFull path to xindy executable.\n",
    "\t\t(Default assumes xindy is on the operating system's path.)\n";

   print "\nMakeindex Options:\n";
   print "(See makeindex documentation for further details on these ";
   print "options.)\n\n";
   print "-c\t\tCompress intermediate blanks.\n";
   print "-g\t\tEmploy German word ordering.\n";
   print "-p <num>\tSet the starting page number to be <num>.\n";
   print "-r\t\tDisable implicit page range formation.\n";
   print "-m <file>\tFull path to makeindex executable.\n",
    "\t\t(Default assumes makeindex is on the operating system's path.)\n";
}

sub VERSION_MESSAGE{

   my $verYear = '';

   if ($version=~/(\d{4})-\d{2}-\d{2}/)
   {
      $verYear = "-$1";
   }

   print "Makeglossaries Version $version\n";
   print "Copyright (C) 2007$verYear Nicola L C Talbot\n";
   print "This material is subject to the LaTeX Project Public License.\n";
}

1;

=head1 NAME

makeglossaries  - Calls makeindex/xindy for LaTeX documents using glossaries package

=head1 SYNOPSIS

B<makeglossaries> [B<-o> I<file>] [B<-q>] [B<-Q>] [B<-k>] [B<-n>]
[B<-s> I<file>] [B<-t> I<file>] [B<-L> I<language>] [B<-c>] [B<-g>] [B<-l>]
[B<-p> I<num>] [B<-r>] [B<-d> I<aux dir>] [B<-m> I<file>] [B<-x> I<file>]
[B<--version>] [B<--help>] I<basename>

=head1 DESCRIPTION

B<makeglossaries> is designed for use with LaTeX documents that
use the glossaries package. The mandatory argument I<basename> should
be the name of the LaTeX document without the .tex extension. 
B<makeglossaries> will read the auxiliary file to determine whether
B<makeindex> or B<xindy> should be called. All the information
required to be passed to the relevant indexing application should
also be contained in the auxiliary file, but may be overridden by
the option arguments to B<makeglossaries>.

=head1 OPTIONS

=over 4

=item B<-q>

Quiet mode. Reduces chatter to standard output.

=item B<-Q>

Silences warning about being unable to fork.

=item B<-k>

Don't try forking with piped redirection. (Lessens the
effect of -q)

=item B<-n>

Print the commands that would normally be executed but don't run them.

=item B<-o> I<file>

Use I<file> as the output file. (Only suitable for documents 
containing a single glossary, otherwise each glossary will be
overridden.)

=item B<-s> I<file>

Use I<file> as the style file. Note that if you use this option,
you need to know whether B<makeindex> or B<xindy> will be called, as
they have different style files.

=item B<-t> I<file>

Use I<file> as the transcript file.

=item B<-l>

Letter ordering.

=item B<-L> I<language>

This option only has an effect if B<xindy> is called. Sets the
language. See B<xindy> documentation for further details.

=item B<-c>

Compress intermediate blanks (B<makeindex> only).

=item B<-g>

Employ German word ordering (B<makeindex> only).

=item B<-p> I<num>

Sets the starting page number to be I<num> (B<makeindex> only).

=item B<-r>

Disable implicit page range formation (B<makeindex> only).

=item B<-d> I<aux dir>

Specify the directory the .aux, .glo etc files are located.
Defaults to the parent directory of the base file I<filename>.

=item B<-m> I<file>

Specify the full path name for B<makeindex> to I<file> in the 
event that B<makeindex> isn't on the operating system's path.

=item B<-x> I<file>

Specify the full path name for B<xindy> to I<file> in the 
event that B<xindy> isn't on the operating system's path.

=item B<--version>

Prints version number and exits.

=item B<--help>

Prints help message and exits.

=back

=head1 REQUIRES

Perl, Getopt::Std, and makeindex or xindy (depending on glossaries
package options).

=head1 LICENSE

This is free software distributed under the LaTeX Project Public 
License. There is NO WARRANTY.
See L<http://www.latex-project.org/lppl.txt> for details.

=head1 AUTHOR

Nicola L. C. Talbot,
L<http://www.dickimaw-books.com/>

=head1 RECOMMENDED READING

The glossaries manual:

	texdoc glossaries

=cut

